Depth Separation with Multilayer Mean-Field Networks

Depth separation -- why a deeper network is more powerful than a shallower one -- has been a major problem in deep learning theory. Previous results often focus on representation power. For example, arXiv:1904.06984 constructed a function that is easy to approximate using a 3-layer network but not approximable by any 2-layer network. In this paper, we show that this separation is in fact algorithmic: one can learn the function constructed by arXiv:1904.06984 using an overparameterized network with polynomially many neurons efficiently. Our result relies on a new way of extending the mean-field limit to multilayer networks, and a decomposition of loss that factors out the error introduced by the discretization of infinite-width mean-field networks.

==> stage-2/stage-2-1.tex <==
\subsection{Stage 2.1 (deprecated)}


\begin{lemma}
  \label{lemma: stage 2.1: E (f* - f) |x| <= log d}
  Suppose that \inductRefS{2} is true at time $t$ and $|\bar{w}_2 \alpha| \le 1 / d^2$. Then we have
  $\E_{\x} \braces{ (f_*(\x) - f(\x)) \norm{\x} } \le - \Theta(\log d)$. 
\end{lemma}
\begin{proof}
  Clear that $\E_{\x} \braces{ f_*(\x) \norm{\x} } = O(1)$. Since $|\bar{w}_2 \alpha| \le 1/d^2$,
  $f \ge \bar{b}_2 / 2 = \Omega(1)$ on $\{ \norm{\x} \le \Theta(1/d^2) \}$. Then, by 
  Lemma~\ref{lemma: input distribution, regularity}, we have
  $
    \E_{\x} \braces{ f(\x) \norm{\x} } 
    = \Omega(1) \E_{\norm{\x} \le \Theta(1/d^2)} \norm{\x}
    = \Omega(\log d). 
  $
  As a result, $\E_{\x} \braces{ (f_*(\x) - f(\x)) \norm{\x} } \le - \Theta(\log d)$. 
\end{proof}



\begin{lemma}[Stage~2.1]
  \label{lemma: stage 2.1: main}
  Suppose that \inductRefS{2} is true throughout Stage~2. Let $T_{2, 1} := \inf\{ t \ge T_1 
  \,:\, \alpha = 1/d^3 \}$. Then, at time $T_{2, 1}$, we have $\alpha = 1/d^3$ and 
  $\bar{w}_2 = \Theta(1/d)$. Moreover, $T_{2, 1} - T_1 \le O\left( \frac{R_{\v_1}^2 \log(d/\eps)}
  {d^{1.5}} \right)$.
\end{lemma}
\begin{proof}
  First, by Lemma~\ref{lemma: stage 2: absorb sigma' into f}, we have
  \[
    \dot{v}_2
    = \E_{\x} \braces{ 
        (f_*(\x) - f(\x) ) F(\x) 
      }
      \pm O\left( d \delta\ps{2}_2  \alpha \log(d/\eps) \right).
  \]
  Hence, 
  \[
    \dot{\bar{w}}_2
    = \E_{\x} \braces{ 
        (f_*(\x) - f(\x) ) \bar{F}(\x) 
      } \alpha
      \pm O\left( d \delta\ps{2}_2 \alpha \log(d/\eps) \right).
  \]
  Similarly, by Lemma~\ref{lemma: stage 2: absorb sigma' into f} and Lemma~\ref{lemma: stage 2: 
  dynamics of alpha}, we have
  \[
    \dot{\alpha}
    = \frac{4 C_\Gamma}{\sqrt{d}} \E_{\x} \braces{ (f_*(\x) - f(\x)) \bar{F}(\x) } \alpha \bar{w}_2
      \pm O\left( 
          \log(d/\eps) \sqrt{d} \delta\ps{2}_2  \alpha \bar{w}_2 
        \right).
  \]
  For notational simplicity, define $A = \E_{\x} \braces{ (f_*(\x) - f(\x)) \bar{F}(\x) } / 2$.
  Here, we add a $1/2$ factor in the definition of $A$ so that we can ignore noise terms. 
  Note that, by Lemma~\ref{lemma: stage 2.1: E (f* - f) |x| <= log d}, $A = -\Theta(\log d)$. As
  a result, 
  \[
    \dot{\bar{w}}_2 = - \Theta(\log d) \alpha
    \quad\text{and}\quad
    \dot{\alpha} = \Theta(\log d) |\bar{w}_2| \alpha.
  \]
  First, for $\bar{w}_2$, we have 
  \[
    \bar{w}_2(T) 
    \le - \Theta\left( (\log d) \alpha(T_1) T \right)
    = - \Theta\left( \frac{(\log d) \sqrt{d}}{ R_{\v_1}^2 } T \right). 
  \]
  Let $T_{\Tmp, 1}$ to be the time needed for $\bar{w}_2$ to reach $-1 / \poly_{\bar{w}_2}(d)$.
  We have
  \[
    T_{\Tmp, 1} \le O\left( \frac{R_{\v_1}^2 }{\sqrt{d} \log(d) \poly_{\bar{w}_2}(d)} \right).
  \]
  Now we consider $\alpha$. First note that at time $T_1 + T_{\Tmp, 1}$, $\alpha = \Theta(\sqrt{d}
  / R_{\v_1}^2)$ still holds. After $T_1 + T_{\Tmp, 1}$, we have $\dot{\alpha} \ge \Theta(\log d)
  / \poly_{\bar{w}_2}(d) \alpha$. Therefore, for any $T > 0$, we have 
  \[
    \alpha(T_1 + T_{\Tmp, 1} + T)
    \ge \Theta\left( \frac{1}{R_{\v_1}^2} \right) 
      \exp\left( \frac{(\log d) T}{\poly_{\bar{w}_2}(d)} \right).
  \]
  Let $T_{\Tmp, 2}$ be the time needed for $\alpha$ to reach $1 / \poly_{\alpha}(d)$. We have
  \[
    T_{\Tmp, 2}
    \le O\left( \log(d/\eps) \poly_{\bar{w}_2}(d) \right). 
  \]
  Meanwhile, at time $T_{2, 1} := T + T_{\Tmp, 1} + T_{\Tmp, 2}$, we have 
  \[
    |\bar{w}_2(T_{2, 1})|
    \le \frac{1}{\poly_{\bar{w}_2}(d)}
      + \Theta\left( (\log d) \alpha(T_{2, 1}) T_{\Tmp, 2} \right)
    \le \frac{1}{\poly_{\bar{w}_2}(d)}
      + \Theta\left( \frac{\log^2(d/\eps) \poly_{\bar{w}_2}(d) }{\poly_{\alpha}(d)} \right).
  \]
  Finally, choose $\poly_{\bar{w}_2} = d$ and $\poly_\alpha(d) = d^3$ and we complete the proof. 
\end{proof}















